Performance Analysis of Optimized Versatile Video Coding Software Decoders on Embedded Platforms

In recent years, the global demand for high-resolution videos and the emergence of new multimedia applications have created the need for a new video coding standard. Hence, in July 2020 the Versatile Video Coding (VVC) standard was released providing up to 50% bit-rate saving for the same video quality compared to its predecessor High Efficiency Video Coding (HEVC). However, this bit-rate saving comes at the cost of a high computational complexity, particularly for live applications and on resource-constraint embedded devices. This paper presents two optimized VVC software decoders, named OpenVVC and Versatile Video deCoder (VVdeC), designed for low resources platforms. They exploit optimization techniques such as data level parallelism using Single Instruction Multiple Data (SIMD) instructions and functional level parallelism using frame, tile and slice-based parallelisms. Furthermore, a comparison in terms of decoding run time, energy and memory consumption between the two decoders is presented while targeting two different resource-constraint embedded devices. The results showed that both decoders achieve real-time decoding of Full High definition (FHD) resolution over the first platform using 8 cores and High-definition (HD) real-time decoding for the second platform using only 4 cores with comparable results in terms of average consumed energy: around 26 J and 15 J for the 8 cores and 4 cores embedded platforms, respectively. Regarding the memory usage, OpenVVC showed better results with less average maximum memory consumed during run time compared to VVdeC.

==> OpenVVC proposal INSA - UPM/acronym.tex <==
\usepackage{glossaries}
\newacronym{ai}{AI}{All Intra}
\newacronym{hevc}{HEVC}{High Efficiency Video Coding}
\newacronym{avc}{AVC}{Advanced Video Coding}
\newacronym{jvet}{JVET}{Joint Video Experts Team}
\newacronym{cfp}{CfP}{Call for Proposal}
\newacronym{alf}{ALF}{Adaptive Loop Filter}
\newacronym{wf}{WF}{Wiener filter}
\newacronym{df}{DBF}{Deblocking Filter}
\newacronym{dsf}{DSF}{Diamond Shape Filter}
\newacronym{sao}{SAO}{Sample Adaptive Offset}
\newacronym{cc}{CCALF}{Cross-Component Adaptive Loop Filter}
\newacronym{aps}{APS}{Adaptation Parameter Set}

\newacronym{mpeg}{MPEG}{Motion Picture Experts Group}
\newacronym{vceg}{VCEG}{Video Coding Experts Group}

\newacronym{mse}{MSE}{Mean Squared Error}
\newacronym{tsmc}{TSMC}{Taiwan Semiconductor Manufacturing Company}

\newacronym{asic}{ASIC}{Application-Specific Integrated Circuit}
\newacronym{fpga}{FPGA}{Field Programmable Gate Array}
\newacronym{jem}{JEM}{Joint Exploration Model}
\newacronym{mts}{MTS}{Multiple Transform Selection}
\newacronym{lfnst}{LFNST}{Low Frequency Non-Separable Transform}
\newacronym{dct}{DCT}{Discrete Cosine Transform}
\newacronym{dst}{DST}{Discrete Sine Transform}
\newacronym{ctc}{CTC}{Common Test Conditions}
\newacronym{fft}{FFT}{Fast Fourier Transform}

\newacronym{simd}{SIMD}{Single Instruction Multiple Data}

\newacronym{sps}{SPS}{Sequence Parameter Set}
\newacronym{psp}{PSP}{Picture Parameter Set}
\newacronym{dsp}{DSP}{Digital Signal Processing}
\newacronym{dft}{DFT}{Discrete Fourier Transform}
%\newacronym{ip}{IP}{Intellectual Property}

%%
\newacronym{qt}{QT}{Quad-Tree}
\newacronym{rdo}{RDO}{Rate Distortion Optimization}
\newacronym{vtm}{VTM}{VVC Test Model}
\newacronym{vhdl}{VHDL}{VHSIC Hardware Description Language}
\newacronym{alm}{ALM}{Adaptive Logic Module}
\newacronym{hw}{HW}{Hardware}
\newacronym{vb}{VB}{Virtual Boundary}
\newacronym{dpb}{DPB}{Decoded Picture Buffer}
\newacronym{mtt}{MTT}{Multi Type Tree}
\newacronym{rd}{RD}{Rate Distortion}
\newacronym{bt}{BT}{Binary Tree}
\newacronym{tt}{TT}{Ternary Tree}
\newacronym{cm}{CM}{Constant Multipliers}
\newacronym{tu}{TU}{Transform Unit}
\newacronym{fps}{fps}{Frame Per Second}
\newacronym{ssd}{SSD}{Sum of Squared Differences}
\newacronym{klt}{KLT}{Karhunen-Loéve Theorem}
\newacronym{nsst}{NSST}{Non-Separable Secondary Transform}
%ù
\newacronym{ra}{RA}{Random Access}
\newacronym{vvc}{VVC}{Versatile Video Coding}

\newacronym{iict}{IICT}{Inverse Integer Core Transforms}
\newacronym{vlsi}{VLSI}{Very Large Scale Integration}
\newacronym{bdr}{BD-BR}{Bj\o ntegaard Delta Rate}
\newacronym{sram}{SRAM}{Static Random Access Memory}

\newacronym{ram}{RAM}{Random-Access Memory}
\newacronym{rom}{ROM}{Read-Only Memory}
\newacronym{rm}{RM}{Regular Multiplier}
\newacronym{mcm}{MCM}{Multiple Constant Multiplier}

\newacronym{dc}{DC}{Design Compiler}
\newacronym{idst}{IDST}{Inverse DST}
\newacronym{idct}{IDCT}{Inverse DCT}

\newacronym{qp}{QP}{Quantization Parameter}
\newacronym{mc}{MC}{Motion Compensation}

\newacronym{cu}{CU}{Coding Unit}
\newacronym{ctu}{CTU}{Coding Tree Unit}
\newacronym{ctb}{CTB}{Coding Tree Block}
\newacronym{vvdec}{VVdeC}{Versatile Video deCoder}
\newacronym{esoc}{ESoC}{Embedded System-on-Chip}
\newacronym{lmcs}{LMCS}{Luma Mapping with Chroma Scaling}
\newacronym{lmp}{LMP}{Luma Mapping}
\newacronym{csp}{CSP}{Chroma Scaling}
\newacronym{cabac}{CABAC}{context adaptive binary arithmetic coding}
\newacronym{ilmcs}{ILMCS}{Inverse Luma Mapping Chroma Scaling}
\newacronym{sse}{SSE}{Streaming SIMD Extensions}
\newacronym{avx}{AVX}{Advanced Vector Extensions}
\newacronym{egpp}{EGPP}{Embedded general purpose processor}
\newacronym{wpp}{WPP}{Wave-front Parallel Processing}
\newacronym{simde}{SIMDe}{SIMDEverywhere}
\newacronym{ep}{EP}{Inter Prediction}
\newacronym{ip}{IP}{Intra Prediction}
\newacronym{tx}{TX}{Inverse Quantization and Transform}
\newacronym{ed}{ED}{Entropy Decoding}
\newacronym{cpu}{CPU}{Central Processing Unit}
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{hd}{HD}{High-definition}
\newacronym{fhd}{FHD}{Full High-definition}
\newacronym{uhd}{UHD}{Ultra High-definition}
